Footballonomics: The Anatomy of American Football; Evidence from 7 years of NFL game data

Do NFL teams make rational decisions? What factors potentially affect the probability of wining a game in NFL? How can a team come back from a demoralizing interception? In this study we begin by examining the hypothesis of rational coaching, that is, coaching decisions are always rational with respect to the maximization of the expected points scored. We reject this hypothesis by analyzing the decisions made in the past 7 NFL seasons for two particular plays; (i) the Point(s) After Touchdown (PAT) and (ii) the fourth down decisions. Having rejected the rational coaching hypothesis we move on to examine how the detailed game data collected can potentially inform game-day decisions. While NFL teams personnel definitely have an intuition on which factors are crucial for winning a game, in this work we take a data-driven approach and provide quantifiable evidence using a large dataset of NFL games for the 7-year period between 2009 and 2015. In particular, we use a logistic regression model to identify the impact and the corresponding statistical significance of factors such as possession time, number of penalty yards, balance between passing and rushing offense etc. Our results clearly imply that avoiding turnovers is the best strategy for winning a game but turnovers can be overcome with letting the offense on the field for more time. Finally we combine our descriptive model with statistical bootstrap in order to provide a prediction engine for upcoming NFL games. Our evaluations indicate that even by only considering a small number of (straightforward) factors, we can achieve a very good prediction accuracy. In particular, the average accuracy during seasons 2014 and 2015 is approximately 63%. This performance is comparable to the more complicated state-of-the-art prediction systems, while it outperforms expert analysts 60% of the time.

==> texfiles/3-model.tex <==
\section{The Irrational Coaching Hypothesis}
\label{sec:2pt-conv}

We begin with examining whether decisions made by coaching staff are always rational.  
In fact, our running hypothesis is: 

\begin{hyp} 
\label{hyp:h1}{\tt [Irrational Coaching]:}
Coaching decisions are not always rational.   
\end{hyp}

We verify the above hypothesis by analyzing the decisions made for the PAT.  
%Before presenting our prediction model, we would like to analyze 
In particular, the dominant decision is to settle for the extra point after a touchdown instead of trying to score more points and attempting a two-point conversion.  
%In particular, 
From the 9,021 touchdowns during the 7 regular seasons that our data span, only 460 of them were followed by a two-point conversion attempt.  
From these, 235 were successful, that is, an overall 51\% success rate.  
On the other hand, from the 8,561 extra point kick attempts, 8,425 were successful, which translates to a 98.4\% success rate.   
If the decision criteria was the success rate, then the extra point kick is clearly the optimal choice! 
However, a game is won by points and not success rates and therefore, the coaching objective is to maximize the (expected) number of points scored.  %we have to base our decision on the expected number of points that we will have with each strategy.  
With the extra point kick, the probability of success is 0.984 and thus, the expected number of points is 0.984.  
On the contrary, with the two-point conversion the success rate is only 0.51 but the expected number of points is 1.02, which is greater than the expected number of points with an extra point kick! 

Of course, not all the teams have the same success rate in the two-point conversions and the extra point kick attempts.  
Figure \ref{fig:2pts} presents the expected benefit in terms of earned points per touchdown $p$ if teams shifted from extra point kick to two-point conversions: 

\begin{equation}
p = 2\cdot \success_{{\tt 2pts}} - 1\cdot \success_{{\tt kick}}
\label{eq:2pts}
\end{equation} 
where $\success_{{\tt 2pts}}$ and $\success_{{\tt kick}}$ are the success rates for the two-point conversions and extra point kicks respectively.  
As we can see not all teams would necessarily benefit from this strategy.  
However, practicing two-point conversion plays can be beneficial in the long term.  
Increasing slightly the success rates can turn to non-negligible point gains.  
In fact, the new rules for the extra point kicks introduced in the last season\footnote{The extra kick is taken from the 15 yard line instead of the 10 yard line.} (2015) has led a statistically significant reduction in $\success_{{\tt kick}}$.  
Table \ref{tab:kick_success} depicts the success rates for the extra point kicks over the years that our dataset spans.  
As one can observe there is a significant drop of approximately 5\% ($p$-value $< 10^{-6}$) in the success rate during the 2015 season! 
On the contrary, there was no impact on the success rate of the two-point conversion attempts (as one might have expected).  
The success rate for 2015 was 1.6\% higher than the yearly average success rate between 2009-2014, however this difference was not statistically significant ($p$-value = 0.4).   
Therefore, it appears a good strategy for the teams to start practicing and attempting two-point conversions, while it is also clear that Hypothesis \ref{hyp:h1} is verified.  

Currently, the decision to attempt a two-point conversion depends mainly on the score differential and the time remaining in the game, two supposedly irrelevant factors as per a rational economic model \cite{thaler2015misbehaving}.  
For instance, when a team scores a touchdown which gives them the lead by one point, it is typical to try for the two point conversion that will potentially give a 3 point lead instead of a 2, hence putting the pressure on the opposing team to score a touchdown to win the game.  
When the touchdown provides a two point lead then things are more complicated and typically teams will attempt the extra point kick.  
What our analysis suggests is that these factors should not impact the decision to attempt a two point conversion, since the expected point benefit is larger regardless of these factors.  
In fact, if a team includes in its playbook the conversion, the success rate $\success_{{\tt 2pts}}$ is also expected to get higher - at least during a transient period - and thus, an even greater benefit is expected.  
Of course at some point the opposing defenses will also adopt and hence, $\success_{{\tt 2pts}}$ will converge to a steady value.    
However, we believe that teams will continue to be conservative, mainly due to the fact in order for the expected outcome to converge to what is predicted by Equation \ref{eq:2pts} a very large number of attempts need to made.  
And while throughout a season this is true, it is not true within a single game where a very small number of attempts will be made by each team (on average 2.5 touchdowns per team per game).  

\section{Winning Factors}
\label{sec:model}

In this section we will analyze the game data using a generalized linear model and in particular logistic regression.  
Let us denote with $\winrv$ the binary random variable that represents that event of winning a game.  
$\winrv = 1$ if the team wins the game and 0 otherwise.  
The output of the logistic regression $\outputvar$ provides us with the probability of this random variable taking the value of 1, i.e., $\outputvar=\Pr[\winrv = 1]$.  
Hence, simply put, $\outputvar$ is the probability of winning.  
The input of this model is a vector $\inputvec$ that includes features that can potentially impact the probability of a team winning.  
With this setting the logistic regression model for $\winrv$ is given by: 

\begin{equation}
\Pr(\winrv=1| \inputvec)= \frac{\exp(\weight^T\cdot\inputvec)}{1+\exp(\weight^T\cdot\inputvec)}
\label{eq:logistic}
\end{equation}

The coefficient vector $\weight$ includes the weights for each individual element of the input vector $\inputvec$, and is estimated using the game data.  
The value of coefficient $\weightel_i$ quantifies the impact that feature $\inputelement_i$ has on the probability of win, while the corresponding $p$-value quantifies its statistical significance.  
The features we use as the input for our model include: 

{\bf  Total offensive yards: }
This feature captures the total yards (rushing and passing) produced by the offense in the game.  

{\bf Penalty Yards: }
This features captures the total yards the team was penalized with.  

{\bf Turnovers: }
This feature captures the total turnovers produced by the team (i.e., how many times the quarterback was intercepted, fumbles recovered by the opposing team and turns on downs).  

{\bf Interceptions: }
This feature represents the total number of interceptions captured by the defense.

{\bf Possession time: }
This feature captures the total ball possession time for the team. 

{\bf Passing-to-Rushing ratio $\ratio$: }
The passing-to-rushing ratio $\ratio$ corresponds to the fraction of offensive yards gained by passing: 

\begin{equation}
\ratio = \dfrac{\textsf{\# of passing yards}}{\textsf{\# of total yards}}
\label{eq:ratio}
\end{equation}

The goal of this feature is to capture the offense's balance between rushing and passing.  
A perfectly balanced offense will have $\ratio=0.5$. 
We would like to emphasize here that $\ratio$ refers to the actual yardage produced and not the passing/rushing attempts.  

Before delving into the details of the descriptive model, we perform some basic analysis that compares the features we will include in the model.  
In particular, we perform a paired t-test for each feature, where each pair corresponds to a specific game.  
More specifically, for each feature $\inputelement_i$, we compare the pairs ($\inputelement_{i,j}^+,~\inputelement_{i,j}^-$), where $\inputelement_{i,j}^+$ ($\inputelement_{i,j}^-$) is the value of $\inputelement_i$ for the winner (loser) of the j$^{th}$ game in our dataset.  
Table \ref{tab:test} depicts the results of the two-sided paired t-tests.    
As we can see all of the differences are significantly different than zero (at the significance level of $\alpha=0.01$).  
Figure \ref{fig:ecdf} further presents the empirical cumulative distribution function (ECDF) for the paired differences for all the features.  
For example, we can see that in only 20\% of the games the winning team had more turnovers compared to the losing team.                        
We further perform the Kolmogorov-Smirnov test for the ECDFs of the considered features for the winning and losing teams.  
The tests reject the null hypothesis at the significance level of $\alpha=0.01$ for all cases, that is, the distribution of the features is statistically different for the winning and losing teams.

Our basic data analysis above indicates that the distribution of the features considered is significantly different for the winning and losing teams.  
To further support this, we use our data to train the logistic regression model and we obtain the results presented in Table \ref{tab:regr}.  
As we can see all the coefficients are statistically significant.  
However, the number of total yards produced by the offense as well as the possession time seem to have the weakest correlation with the probability of winning a game.  
On the contrary committing turnovers quickly deteriorates the probability of winning the game and the same is true for an unbalanced offense.  

While the direction of the effects for these variables are potentially intuitive and straightforward for the coaching staff of NFL teams, the benefit of our quantifying approach is that it assigns specific magnitude to the importance of each factor.  
For example, if we want to increase the probability of winning by 10\% the team should decrease the turnovers it commits (keeping all else constant) by approximately 20\% on average.   %either increase the total yards gained by approximately 19\% on average (keeping all else equal), or increase the possession time by 11\% on average (keeping all else equal).  
On the contrary, if the team was working on reducing its penalty yards, the same effect (i.e., increase by 10\% the probability of winning) would require a reduction in the penalty yardage by approximately 72\% on average.  
Hence, while all of the factors considered are statistically significant, some of them appear to be much more important and potential parts of the game a team could work on.  

More importantly though we would like to reflect on how one should interpret and use these results.  
For example, one could be tempted to focus on the feature with the coefficient with maximum absolute magnitude, that is, ratio $\ratio$ and conclude that making $\ratio = 0$, that is, calling only run plays will increase the probability of win.  
However, this is clearly not true as every person with basic familiarity with American football should know.  
At the same time the logistic regression model is not contradicting itself! 
What happens is that the model developed - similar to any data driven model - is {\em valid} only for the range of values that the input variables cover\footnote{In particular, the range that covers the majority of the values of the input variables (e.g., 95\%).}.  
Outside of this range, the (generalized) linear trend might still hold or not (which is most probably the case for $\ratio$).  
Figure \ref{fig:quant-ratio} depicts the distribution of ratio $\ratio$ for the winning and losing teams.  
As we can see our data cover approximately the range $\ratio\in[0.3, 0.98]$ and the trend should only be considered valid within this range (and potentially within a small $\epsilon$).  
It is interesting also to observe that the mass of the distribution for the winning teams is concentrated well above $\ratio = 0.5$, with the maximum density observed for $\ratio \approx 0.64$.  
We also present at the same figure a table with the range that our features cover for both winning and losing teams.   
Furthermore, the logistic regression model captures merely correlations (rather than cause-effect relations). 
Given that some of the features are also correlated themselves (see Figure \ref{fig:corr}) and/or are result of situational football makes it even harder to identify real causes.  
For instance, there appears to be a small but statistically significant negative correlation between ratio $\ratio$ and possession time.  
Furthermore, a typical tactic followed by teams leading in a game towards the end of the fourth quarter is to run the clock out by calling run plays.  
This will lead to a reduced ratio $\ratio$ as compared to the counterfactual $\ratio$ expected if the team continued its original game-plan and hence, might artificially deflate the actual contribution of $\ratio$ on the probability of winning.  
Similarly, teams that are behind towards the end of the game will typically call plays involving long passes in order to cover more yardage.  
However, these plays are also more risky and will lead to turnovers more often, therefore, inflating the impact of turnovers in the probability of win.  
Nevertheless, this is always a problem when a field experiment cannot be designed and only observational data are available.  
In conclusion, our model provides quantifiable, actionable, insights but they need to be carefully interpreted when designing play actions based on it.  
  



==> texfiles/4-predict.tex <==
\section{Predictive Model}
\label{sec:predict}

We now turn our attention on how we can use the above model in order to predict the outcome of a future game.  
In a realistic setting, in order to be able to apply the logistic regression model we trained with the historical data we will need to provide the team statistics input required.  
This is by itself a separate prediction problem.  
Hence, we begin by evaluating the prediction performance of the logistic regression model itself using traditional machine learning evaluation methods.  
In particular, we evaluate the accuracy prediction of our model through cross validation.  
In this way we do not need to predict the value of the features but we explore the accuracy of the pure logistic regression model.   
Using 10-fold cross validation we obtain an accuracy of {\bf 80.45\%} $\pm$ {\bf 0.9\%}.  
To reiterate this performance is conditional to the input features being known! 
However, how can we predict these features?  
After all a realistic system will need to do this.  
Simply put, a prediction system will need to first predict the two teams statistics/features (i.e., total yards, penalty yards, etc.) and then use the logistic regression model to predict the winning team.  

The most straightforward way for this task is to use historic game data from the current season and calculate descriptive statistics such as the mean or the median of each feature.  
The problem with this approach is that the NFL season is fairly small (compared to other sports) and hence, descriptive statistics such as the mean and the median might not be appropriate.  
Therefore, we propose to utilize statistical bootstrap in order to resample with replacement $\boots$ times the empirical distribution for each one of the features from the observed sample.  
%Then we will utilize these distributions to ``simulate'' the performance of each team and provide a confidence interval for the probability of win for each of the teams.  
Figure \ref{fig:system} illustrates the components of our prediction engine.  

More specifically, the first part of the prediction engine obtains three inputs; (i) historical information for games of the current season, (ii) the number of bootstrap samples $\boots$ to obtain and (iii) the correlation matrix between the six features considered.  
In particular, for every team $T$ we have a matrix ${\bm M}_T$ each row of which represents a game in the current season, while the columns correspond to the six different features.  
In the case of ``simple'' bootstrapping we would uniformly at random select for each feature one row (i.e., one of the past performances of the team with respect to this feature) and hence, we would obtain a resampled vector ${\bm x}_T^i$ that represents a potential performance for $T$ given its past.  
However, there are two factors that we need to take into consideration.  
Firstly, more recent games might be more representative of recent adjustments (or roster losses due to injuries) as compared to performances during the first weeks of the season.  
In order to control for this, instead of sampling the rows of ${\bm M}_T$ for every feature uniformly at random, we bias the sampling probabilities to favor the last $k$ games of the team.  
Secondly, sampling the features independently can lead to vectors ${\bm x}_T^i$ that do not exhibit the correlations between the features that are present in the actual data.  
Figure \ref{fig:corr} represents the correlations between the different pairs of features.  
For example, as we can see the total yards and the possession time exhibit a medium to strong level of correlation.  
This means that when we sample for the total yards of the i$^{th}$ bootstrap sample, we should not sample the possession time independently, but rather select the possession time from the same game/row of ${\bm M}_T$.  
This essentially mimics the block bootstrapping approach \cite{kunsch89} used for time-series data in order to keep the dependencies between consecutive time-points.  
The rest of the correlations between the features are fairly weak (and some also insignificant) and hence, we proceed as normal with the rest of the features.  

Once bootstrapping is completed, its output is essentially a set of potential future performances for each team as captured through the feature vectors.  
Simply put for each of the two competing teams we have bootstrapped vectors ${\bm x}_1^1, {\bm x}_1^2,\dots,{\bm x}_1^{\boots}$ and ${\bm x}_2^1, {\bm x}_2^2,\dots,{\bm x}_2^{\boots}$ respectively.  
These vectors then form the input in our logistic regression model (see Section \ref{sec:model}) through which we obtain a set of winning probabilities for each team, that is, $\mathcal{P}_1 = \{\Pr(\winrv_1=1|{\bm x}_1^1),\dots,\Pr(\winrv_2=1|{\bm x}_1^{\boots})\}$ and $\mathcal{P}_2 = \{\Pr(\winrv_2=1|{\bm x}_2^1),\dots,\Pr(\winrv_2=1|{\bm x}_2^{\boots})\}$.  
Once we obtain these probabilities sets, we finally perform a hypothesis test to identify whether the two sets represent probabilities that are statistically different at a predefined significance level $\alpha$: 

\vspace{-0.15in}
\begin{eqnarray}
H_0: & \overline{\mathcal{P}_1} = \overline{\mathcal{P}_2} \label{eq:null}\\
H_1: & \overline{\mathcal{P}_1} \neq \overline{\mathcal{P}_2} \label{eq:alt}
\end{eqnarray}

If the null hypothesis is rejected, then the sign of the difference $\overline{\mathcal{P}_1}-\overline{\mathcal{P}_2}$ will inform us about the team most probable to win the matchup.  
We have evaluated our prediction engine with the 5 last weeks of the 2015 regular season.  
In particular, we build our logistic regression model using the game data for the seasons 2009-2014.  
We further set $\boots = 1,000$, $k=5$ and $\alpha  = 0.05$.  
Table \ref{tab:prediction} presents the number of correct game outcomes predicted by our engine (there are 16 games every week).  
While these numbers might not appear impressive, they are on average better than approximately 60\% of the expert predictions.  % \cite{nfl-expert}! 
The expert predictions we considered form a very good baseline since they include the forecasts of sports analysts from major networks (ESPN, NFL network, CBS and FOX sports) \cite{nfl-expert}.  

We further present in Figure \ref{fig:accuracy} the actual accuracy of our prediction engine for the seasons 2014 and 2015 for weeks 8-17.  
As we can see in both seasons the prediction accuracy in weeks 13-17 is higher as compared to weeks 8-12.  
The reason for that is that in weeks 13-17 there is a greater amount of historic performance data for bootstrap to work with.  
We further observe that the prediction accuracy in 2015 season is worse as compared to that of the 2014 season.  
We speculate that this is due to the much higher variability in the performance of the teams during 2015. 

\subsection{Discussion and Limitations}
\label{sec:disc}

In our evaluation, we focused on the last 5 weeks of the 2015 regular season.  
The reason for this is that in Week 13 we have a good amount of historic information from the season in order to provide an accurate prediction.  
Earlier in the season this information is even more sparse and our system's accuracy is expected to exhibit high variance.  
With respect to the performance of our prediction engine we would like to emphasize on the fact that it is very impressive if one considers that we do not account for game-specific information (e.g., injured players, teams resting players during the last week, etc.).  
Even without considering such information the system performs on average better than 60\% of the experts, who are taking into consideration these signals.  
Hence, our system in its current form can be considered as providing an {\em anchoring} probability \cite{kahneman1973psychology} from which an expert can adjust his/her prediction using game-specific information.  
Furthermore, there is room for further improving this anchoring probability.  
In particular, one of the limitations of our system is that currently it does not incorporate any information for the schedule strength of teams.  
Simply put, when performing the bootstrap for the future performance of team $T$ we just extrapolate from the older performance of $T$ without considering the strength of the teams that it has played against.  
For example, in the 2014 NFL season the winner of NFC South (Carolina Panthers) had a percentage record less than 0.5.  
This means that Carolina had faced mainly teams with a losing record and hence, the corresponding team statistics might have been inflated as a result of the bootstrap process described above.  
However, our engine is easily adoptable to account for this.  
In particular, let us consider that we want to estimate the performance of team $T_1$ against $T_2$.  
In order to account for the strength of $T_2$, we can bias the re-sampling probabilities based on the propensity score \cite{austin2011introduction} of the set of teams $\mathcal{T}$ that $T_1$ has faced in the past. %, $\mathcal{T}$.  
The propensity score is mainly used as a quasi-experimental technique, in order to match a treated sample with an untreated observational set based on a set of observable cofounders.  
In our setting, the propensity score $\pi_i$ for $T_i \in \mathcal{T}$ will simply provide as with the ``similarity'' of $T_i$ with $T_2$.  
Consequently, the resampling probability for $T_i$ will be proportional to $\pi_i$. 
%Considering this interactions is part of our future work and we expect this to further improve the performance of our prediction engine.




==> texfiles/7-concl.tex <==
\section{Conclusions}
\label{sec:conclusions}

In this work we collected and analyzed game data from the last 7 seasons of the National Football League.  
We first explored the running hypothesis that coaching decisions are many times irrational and do not follow the strategy that would be predicted from a rational agent.  
To verify this hypothesis we used evidence from the behavior of a team for the PAT.  
We find that while currently the decision to run a two-point conversion depends mainly on the time remaining in the game and the score differential, this should not be the case, since the expected point benefit is higher as compared to the extra point kick that is chosen 95\% of the times.  
We then explored the impact of some basic factors on the probability of a team winning the game through a logistic regression model.  
This quantification is important and can potentially help coaching staff in decision making.  
We also provide guidelines on how the model and its findings should be interpreted.  
%Furthermore, we challenged the decision of the teams to settle for an extra point kick after a touchdown instead of a two-point conversion.  
%While not all of the teams will benefit from this strategy, this might change with the new rules for the extra point kick introduced this year by NFL.  
Finally, we designed a game prediction engine that utilizes statistical bootstrap and the logistic regression model we developed.  
The novelty of the system resides on the statistical bootstrap module that aims into alleviating the impact of the small (for statistical purposes) NFL season.   
Our evaluations indicate that our system can provide a very good accuracy prediction and it can certainly be used as an anchoring probability that can then be adjusted by considering matchup-specific information.  

==> texfiles/8-figuresAndTables.tex <==
\section{Figures and Tables}

 \begin{figure}[h]
\begin{center}
\includegraphics[scale=0.26]{figures/2pts}
\caption{Different teams have different expected point gains based on the corresponding success rates $\success_{{\tt2pts}}$ and $\success_{{\tt kick}}$.  On the top of each bar we also present the number of times that the corresponding team attempted a two-point conversion in our dataset.  Pittsburgh Steelers and Chicago Bears appear to have to gain the most from switching to two-point conversions.  In fact, half of the Steeler's two-point conversion attempts in the dataset happened during the 2015 regular season.  The largest expected gain is observed for San Diego.  However, the Chargers have only tried the two-point conversion 6 times and we cannot consider the corresponding success rate statistically representative.}
\label{fig:2pts}
\end{center}
\end{figure}

\begin{table}[h]
\scriptsize
  \begin{center}
  
    \begin{tabular}{l|c|c}
    \toprule
\bf Year & \bf $\success_{{\tt kick}}$ & \bf $\success_{{\tt 2pt}}$ \\
      \midrule
%Intercept &  -3.250511$^{***}$\\
2009 & 0.9814 & 0.4426\\
2010 & 0.9884 & 0.5471\\
2011 & 0.9942 & 0.5 \\
2012 & 0.9935 & 0.55\\
2013 & 0.9960 & 0.4929\\
2014 & 0.9926  & 0.5161\\
2015 & {\bf 0.9416} & 0.5247\\
\bottomrule
    \end{tabular}
    \vspace{0.2cm}
       \caption{The new PAT rules introduced in 2015 have led to significant drop of the success rate of the extra point kick by approximately 5\% ($p$-value $< 0.001$). On the contrary, there is no impact (as expected) on the two-point conversion success rate.  }
    \label{tab:kick_success}
  \end{center}
\end{table}

\begin{table}[h]
\scriptsize
  \begin{center} 
    \begin{tabular}{l|c}
    \toprule
			\bf Feature & \bf Average paired difference \\
      \midrule
%Intercept &  -3.250511$^{***}$\\
Total Yards & 50.95257 $^{***}$\\
Penalty Yards & -3.09375$^{**}$\\
Turnovers & -1.049665$^{***}$\\
Interceptions & 0.390625$^{***}$ \\
Possession Time (sec) & 214.7573$^{***}$ \\
$\ratio$ &  -0.05496846$^{***}$ \\
\bottomrule
    \end{tabular}
    \vspace{0.2cm}
       \caption{Paired t-test for the considered features. The difference represents $\overline{\inputelement_{i,j}^+}-\overline{\inputelement_{i,j}^-}$. Significance codes:   \\ 0 '$^{***}$'   0.01 '$^{**}$'   0.05 '$^{*}$'   0.1 '$.$'   1 ' '.}
    \label{tab:test}
  \end{center}
\end{table}

 \begin{figure}[h]
\begin{center}
\includegraphics[scale=0.8]{figures/ecdf}
\caption{Empirical cumulative distribution function for the differential of each game feature.  Not only the paired means of the features are statistically different but the corresponding ECDFs for the winning and losing teams are statistically different as well (at the significance level $\alpha=0.01$) based on the Kolmogorov-Smirnov test.}
\label{fig:ecdf}
\end{center}
\end{figure}



\begin{table}[h]
\scriptsize
  \begin{center}
    \begin{tabular}{l|c}
    \toprule
			\bf Feature & \bf Coefficient \\
      \midrule
%Intercept &  -3.250511$^{***}$\\
Total Yards & 0.007716$^{***}$\\
Penalty Yards & -0.012323$^{***}$\\
Turnovers & -0.889084$^{***}$\\
Interceptions & 0.654004$^{***}$ \\
Possession Time & 0.002199$^{***}$ \\
$\ratio$ &  -3.142612$^{***}$ \\
\bottomrule
    \end{tabular}
    \vspace{0.2cm}
       \caption{Coefficients of our logistic regression model for the random variable $\winrv$. Significance codes: 0 '$^{***}$'   0.01 '$^{**}$'   0.05 '$^{*}$'   0.1 '$.$'   1 ' '.}
    \label{tab:regr}
  \end{center}
\end{table}

 \begin{figure}[h]
\begin{center}
\includegraphics[scale=0.8]{figures/quantiles-ratio}
\caption{Our model is trained within the range of input variable values on the left table.  The right table presents the probability density function for $\ratio$ for the winning and losing instances respectively. }
\label{fig:quant-ratio}
\end{center}
\end{figure}

 \begin{figure}[h]
\begin{center}
\includegraphics[scale=0.4]{figures/corr}
\caption{Correlations between the different features considered.  Insignificant correlations ($p$-value $> 0.05$) are crossed out.}
\label{fig:corr}
\end{center}
\end{figure}



 \begin{figure}[h]
\begin{center}
\includegraphics[scale=0.8]{figures/predict}
\caption{The proposed prediction engine consists of 3 modules; a bootstrap module, a logistic regression module and a statistical test module.  }
\label{fig:system}
\end{center}
\end{figure}


\begin{table}[h]
\scriptsize
  \begin{center}
    \begin{tabular}{l|c}
    \toprule
			\bf Week & \bf \# of correct predictions \\
      \midrule
%Intercept &  -3.250511$^{***}$\\
13 & 10\\
14 & 8\\
15 & 13\\
16 & 8 \\
17 & 9 \\
\bottomrule
    \end{tabular}
    \vspace{0.2cm}
       \caption{The prediction accuracy of our system outperforms on average 60\% of the expert predictions.}
    \label{tab:prediction}
  \end{center}
\end{table}

 \begin{figure}[ht]
\begin{center}
\includegraphics[scale=0.35]{figures/predict_accuracy.pdf}
\caption{The performance of our prediction engine is better during the last part of the season, since bootstrap has more performance information about the teams to work with.}
\label{fig:accuracy}
\end{center}
\end{figure}


